Optimizing fairness tradeoffs in machine learning with multiobjective meta-models

Improving the fairness of machine learning models is a nuanced task that requires decision makers to reason about multiple, conflicting criteria. The majority of fair machine learning methods transform the error-fairness trade-off into a single objective problem with a parameter controlling the relative importance of error versus fairness. We propose instead to directly optimize the error-fairness tradeoff by using multi-objective optimization. We present a flexible framework for defining the fair machine learning task as a weighted classification problem with multiple cost functions. This framework is agnostic to the underlying prediction model as well as the metrics. We use multiobjective optimization to define the sample weights used in model training for a given machine learner, and adapt the weights to optimize multiple metrics of fairness and accuracy across a set of tasks. To reduce the number of optimized parameters, and to constrain their complexity with respect to population subgroups, we propose a novel meta-model approach that learns to map protected attributes to sample weights, rather than optimizing those weights directly. On a set of real-world problems, this approach outperforms current state-of-the-art methods by finding solution sets with preferable error/fairness trade-offs.

==> tables/tradeoffs.tex <==
% \begin{tabularx}{\columnwidth}{}
%     Metric  &   FNR     & Calibration   & PPV   &   NPV \\
%     FPR     &   \checkmark  &   
%     \\
%     FNR
%     \\
%     Calibration
%     \\
%     PPV
%     \\
%     NPV 
